Training Normalizing Flows with the Information Bottleneck for Competitive Generative Classification

The Information Bottleneck (IB) objective uses information theory to formulate a task-performance versus robustness trade-off. It has been successfully applied in the standard discriminative classification setting. We pose the question whether the IB can also be used to train generative likelihood models such as normalizing flows. Since normalizing flows use invertible network architectures (INNs), they are information-preserving by construction. This seems contradictory to the idea of a bottleneck. In this work, firstly, we develop the theory and methodology of IB-INNs, a class of conditional normalizing flows where INNs are trained using the IB objective: Introducing a small amount of {\em controlled} information loss allows for an asymptotically exact formulation of the IB, while keeping the INN's generative capabilities intact. Secondly, we investigate the properties of these models experimentally, specifically used as generative classifiers. This model class offers advantages such as improved uncertainty quantification and out-of-distribution detection, but traditional generative classifier solutions suffer considerably in classification accuracy. We find the trade-off parameter in the IB controls a mix of generative capabilities and accuracy close to standard classifiers. Empirically, our uncertainty estimates in this mixed regime compare favourably to conventional generative and discriminative classifiers.

==> 01_introduction_OLD.tex <==
The distinction between discriminative and generative classifiers (DCs vs. GCs) is fundamental to machine learning.
DCs directly predict posterior class probabilities $p(Y|X)$, where  $X$ and $Y$ denote input and output variables respectively.
GCs instead model the joint probability $p(X,Y)$, usually as a product of class priors $p(Y)$ and conditional data likelihoods $p(X|Y)$.
They are able to generate synthetic data, and posterior class probabilities can simply be inferred by Bayes' rule $p(Y|X)=p(X|Y)p(Y) / \mathbb{E}_{p(Y)}\left[p(X|Y)\right]$.

DCs optimize prediction performance directly and therefore achieve better results in this respect.
However, their models for $p(Y|X)$ tend to be most accurate near decision boundaries (where it matters), but deteriorate away from them (where deviations incur no noticeable loss).
Consequently, they are poorly calibrated \citep{guo2017calibration} and out-of-distribution data can not be recognized at test time \citep{ovadia2019can}.
In contrast, GCs model full likelihoods $p(X|Y)$ and thus implicitly full posteriors $p(Y|X)$, which leads to the opposite behavior -- better predictive uncertainty at the price of reduced accuracy.

In practice, models trained in a purely generative way (in particular with maximum likelihood), achieve highly unsatisfactory accuracy,
so that some recent work has called into question the overall effectiveness of GCs \citep{fetaya2019conditional, nalisnick2018deep}.
Others have introduced different architectures and augmented losses \citep{jacobsen2018excessive, DBLP:conf/icml/NalisnickMTGL19},
that lead to an improvement of the discriminative capabilities.
In-depth studies of the ideal cases \citep{Lasserre2007GenerativeOD, DBLP:books/lib/Bishop07} revealed the existence of a trade-off, 
controlling the balance between discriminative and generative performance.
The existence of a trade-off is not self evident, as in principle, a more accurate generative model should also lead to better classification.

%\todoLA{(a) why is no-one using the Bishop-net? ($\rightarrow$ impractical training perhaps) (b) how do hybrid models fit in the picture? ($\rightarrow$ not proper gen. classifier bishop says)}

%- how does the tade off work?

%- bishop says it's no good changing the loss like this (`not .. a well-defined model')

%``not derived by maximizing the distribution of a well-defined model'' \citep[p.~7]{Lasserre2007GenerativeOD}.

%We argue in the following that these works may be overly pessimistic, as they do not consider alternative training methods.
%\todoLA{mention `broken' DIGLM loss. In the cases where it works (DIGLM), the loss does not correspond to the claimed loss. Bishop says "Unfortunately, this criterion was not derived by maximizing the distribution of a well-defined model"}
%
We propose the Information Bottleneck (IB) objective \citep{tishby2000information} as an alternative viewpoint of this phenomeneon, 
when applied to generative classification.
%As an alternative, we apply the Information Bottleneck (IB) objective \citep{tishby2000information} to generative classification.
IB formulates the discriminative/generative trade-off in a very general information-theoretic form:
It postulates existence of a latent space $Z$, where all information flow between $X$ and $Y$ is channeled through (hence the method's name).
In order to optimize predictive performance, IB attempts to maximize the mutual information $I(Y,Z)$ between $Y$ and $Z$.
Jointly, it strives to minimize the mutual information $I(X,Z)$ between $X$ and $Z$, forcing the model to ignore irrelevant aspects of $X$, which do not contribute to classification performance and only increase the potential for overfitting. 
The objective can therefore be expressed as
\begin{equation} \label{eq:IB-loss}
    \mathcal{L}_\mathrm{IB} = I(X, Z) - \beta I(Y, Z) \ .
\end{equation}

\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{\input{figures/INN-basic.tex}}
    \caption{Our generative classifier as the Information Bottleneck Invertible Neural Network (IB-INN).}
    \label{fig:INN-basic}
    \vspace{-5mm}
\end{figure}
Unfortunately, practical application of IB as a loss function is difficult because existing estimators for mutual information (MI) are not sufficiently reliable in high dimensions. 
The Variational Information Bottleneck \citep[VIB,][]{DBLP:conf/iclr/AlemiFD017, kolchinsky2017nonlinear} provides a feasible approximation in form of an upper bound for IB, which however does not work as well as the asymptotically exact solution presented in this work.

Using Invertible Neural Networks (INNs), we can, for the first time, train generative classifiers directly with the IB objective, cf.~Fig. \ref{fig:INN-basic}.
This major advance arises from two critical properties of this network type: 
(i) the transformation between $X$ and $Z$ has a tractable Jacobian determinant,
and (ii) the latent space $Z$ can be shaped as a Gaussian Mixture Model (GMM).
As a result, the IB objective is analytically expressible in terms of the change-of-variables formula, allowing for standard gradient descent training without additional approximations. 
%\todoLA{specify more closely what we mean. true MI of the data is just a fixed number, we mean generator MI, strongly consistent, asymptotically reaches data-MI}
Moreover, properties (i) and (ii) facilitate latent space exploration which enables out-of-distribution detection and the analysis of class similarities.
The trade-off parameter $\beta$ occurring in the IB loss (\ref{eq:IB-loss}) allows us to explicitly alter the trade-off between our model's classification performance and it's generative modeling capabilities.
When $\beta$ is adjusted properly, our experiments reveal that IB-INNs simultaneously exhibit high predictive accuracy, well calibrated uncertainties and allow to reliably detect out-of-distribution examples.

To summarize, we combine two concepts -- the Information Bottleneck (IB) objective and Invertible Neural Networks (INNs) -- into a new generative classifier type called IB-INN. Our contributions are as follows:
\begin{itemize}[itemsep=2pt,parsep=2pt,topsep=0pt, partopsep=0pt]
    \item We derive an asymptotically exact formulation of the IB loss for a special GC type by utilizing INNs.
    \item We show experimentally that our models outperform existing GCs on CIFAR10/100 in terms of classification error, and incur at worst minor degradation relative to feed-forward DCs.
    \item We demonstrate good uncertainty quantification in terms of accurate posterior calibration and reliable outlier detection.
    %\item We demonstrate that IB-INNs possess superior uncertainty quantification and outlier detection capabilities compared to alternative models of comparable complexity. 
    %\item We show experimentally that our model incurs only minor degradation in classification accuracy relative to standard feed-forward DCs.
\end{itemize}

\begin{figure}
    \centering
    \resizebox{0.9\linewidth}{!}{\input{figures/generative-classifier.tex}}
    \caption{Illustration of the latent output space of a generative classifier.
    The two class likelihoods for $Y=\{1,2\}$ are parameterized by their means $\mu_{\{1,2\}}$.
    The dotted line represents the decision boundary between the two classes. A confident, an uncertain, and an out-of-distribution sample is illustrated.\vspace{-0.3cm}}
    \label{fig:illust_generative_classifier}
\end{figure}

%\begin{table*}
%\caption{Comparing different models:
%Discriminative classifiers (DCs), Generative classifiers (GCs), Variational Information Bottleneck (VIB), and our Information Bottleneck Invertibel Neural Network (IB-INN).
%\vspace{-0.2cm}
%}
%\centering
%\resizebox{\textwidth}{!}{
%\begin{tabular}{ll|c c c c}
%& & Standard DCs & Standard GCs & VIB & IB-INN (ours)\\
%\hline
%{I.} & Classification Performance &  \tabyes & \tabno & \tabyes & \tabyes \\
%{II.} & Intrinsically well calibrated (i.e.~good Uncertainties) &  \tabno & \tabsoso & \tabno & \tabyes \\
%{III.} & Out-of-Distribution (OoD) detection &  \tabno & \tabyes & \tabno & \tabyes \\
%{IV.} & Generative Model &  \tabno & \tabyes & \tabno & \tabyes \\
%{V.} & Controllable trade-off between I and II,III,IV above & \tabno & \tabsoso & \tabyes & \tabyes 
%\end{tabular}
%}
%\vspace{-0.5cm}
%\end{table*}


==> 04_results_table_OLD.tex <==
\begin{table*}
\caption{
\todoLA{cifar 100 and mnist: see appendix}
Results on the CIFAR10 dataset.
All models have the same number of parameters and were trained with the same hyperparameters.
All values except entropy and overconfidence are given in percent.
The arrows indicate whether a higher or lower value is better. 
The prediction entropy of the model trained with standard class-NLL is not taken into account, 
because the entropy is equally high on in-distribution data due to the poor classification performance.
The OoD detection score for VIB is also not taken into account, see text. 
}
\label{tab:results_cifar10}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l"r"r"r|rrr"r|rrrr"r|rrrr}
\Large \bf CIFAR10 & Classif. &
\multicolumn{4}{c"}{Calibration error ($\downarrow$)} & 
\multicolumn{5}{c"}{OoD prediction entropy ($\uparrow$)} & 
\multicolumn{5}{c}{OoD detection score ($\uparrow$)} \\
& err. ($\downarrow$)&
{\tiny Geo.~mean} & {\tiny Expec.} & {\tiny Max} & {\tiny Overc.} & 
{\tiny Geo.~mean} & {\tiny RGB-rot} & {\tiny Draw} & {\tiny Noise} &{\tiny ImgNet}& 
{\tiny Geo.~mean} & {\tiny RGB-rot} & {\tiny Draw} & {\tiny Noise} &{\tiny ImgNet}\\
\thickhline %& & & & \\
IB-INN (ours, $\tilde \beta = 1$) &
 9.88 &
 \bf 1.969 & 0.93 & \bf 8.20 & \bf 0.00 & 
   \bf 0.865 & \bf 0.86     & \bf 1.07     & \bf 0.59     & \bf 1.02    &
   54.03 & \bf 86.5     & 21.3     & \bf 86.3     & 53.6    
\\ IB-INN, only $\mathcal{L}_Y$ (\small $\tilde \beta \rightarrow \infty$) &
 8.29 &
 6.690 & 1.22 & 23.81 & 10.32 &  
   0.587 & 0.55     & 0.68     & 0.43     & 0.74    &
   \bf 58.72 & 59.7     & \bf 96.4     & 50.9     & 40.6    
\\ IB-INN, only $\mathcal{L}_X$ ($\tilde \beta = 0$) &
 -- &
 -- & -- & -- & -- & 
   -- & --     & --     & --     & --  &
   44.68 & 79.3     & 12.1     & 80.4     & 51.9    
\\ \hline Class-NLL &
 84.98 &
 62.016 & 11.21 & 86.16 & 247.00 & 
   \it (1.067) & \it (1.03     & \it 1.22     & \it 0.97     & \it 1.06)&
   48.55 & 80.2     & 18.6     & 71.6     & 52.0    
\\ Class-NLL (regularized)&
 20.57 &
 24.176 & 3.93 & 20.30 & 177.33 & 
   0.002 & 0.00     & 0.00     & 0.00     & 0.00&
   48.95 & 82.0     & 16.1     & 79.1     & \bf 54.9    
\\ \hline VIB ($\tilde \beta = 1$)&
7.29 &
4.466 & 0.68 & 27.83 & 4.71 & 
0.342 & 0.35     & 0.38     & 0.19     & 0.52&
\it (47.38) & \it (46.4     & \it 52.2     & \it 50.0     & \it 41.7)    
\\ Standard ResNet &
\bf 6.76 &
5.656 & 0.73 & 40.61 & 6.12 &
0.344 & 0.35     & 0.44     & 0.18     & 0.51  &
-- & --     & --     & --     & --    
\\ i-RevNet &
9.09 &
2.224 & \bf 0.54 & 14.78 & 1.37 & 
0.611 & 0.74     & 0.90     & 0.25     & 0.82 & 
-- & --     & --     & --     & --   

%\input{04_results_table_cifar100.tex}
\end{tabular}
}
\end{center}

\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% ALL RESULTS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INI experiments_configs/cifar10/ensemble/full_model_ensemb_0.ini
% ACC     90.1242
% ACC ERR 9.8758
% LATEX 9.88 &
% XCE     ECE       MCE       OVC       
% XCE     0.931643  8.199872  0.000000  
% XCE GM  1.969479
% XCE GMO 0.000000
% LATEX 1.969 & 0.93 & 8.20 & 0.00 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     86.5296     21.2848     86.2976     53.6281     
% AUC ERR 13.4704     78.7152     13.7024     46.3719     
% ENT     0.8637      1.0681      0.5945      1.0224      
% AUC GM  54.032637
% ENT GM  0.865337
% LATEX   54.03 & 86.5     & 21.3     & 86.3     & 53.6    &
% LATEX   0.865 & 0.86     & 1.07     & 0.59     & 1.02    
% 
% INI experiments_configs/cifar10/ablations/no_nll.ini
% ACC     91.7067
% ACC ERR 8.2933
% LATEX 8.29 &
% XCE     ECE       MCE       OVC       
% XCE     1.218549  23.809524 10.320350 
% XCE GM  6.690036
% XCE GMO 6.690036
% LATEX 6.690 & 1.22 & 23.81 & 10.32 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     59.6836     96.3890     50.8574     40.6290     
% AUC ERR 40.3164     3.6110      49.1426     59.3710     
% ENT     0.5504      0.6769      0.4293      0.7427      
% AUC GM  58.717585
% ENT GM  0.587067
% LATEX   58.72 & 59.7     & 96.4     & 50.9     & 40.6    &
% LATEX   0.587 & 0.55     & 0.68     & 0.43     & 0.74    
% 
% INI experiments_configs/cifar10/ablations/beta0.ini
% ACC     9.9960
% ACC ERR 90.0040
% LATEX 90.00 &
% XCE     ECE       MCE       OVC       
% XCE     17.779821 89.830383 266.649039
% XCE GM  75.236620
% XCE GMO 75.236620
% LATEX 75.237 & 17.78 & 89.83 & 266.65 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     79.2752     12.0569     80.4013     51.8599     
% AUC ERR 20.7248     87.9431     19.5987     48.1401     
% ENT     0.0081      0.0029      0.0171      0.0033      
% AUC GM  44.680378
% ENT GM  0.006017
% LATEX   44.68 & 79.3     & 12.1     & 80.4     & 51.9    &
% LATEX   0.006 & 0.01     & 0.00     & 0.02     & 0.00    
% 
% INI experiments_configs/cifar10/ablations/class_nll.ini
% ACC     15.0240
% ACC ERR 84.9760
% LATEX 84.98 &
% XCE     ECE       MCE       OVC       
% XCE     11.208226 86.155202 246.996069
% XCE GM  62.015731
% XCE GMO 62.015731
% LATEX 62.016 & 11.21 & 86.16 & 247.00 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     80.1612     18.6372     71.5678     51.9762     
% AUC ERR 19.8388     81.3628     28.4322     48.0238     
% ENT     1.0346      1.2152      0.9724      1.0589      
% AUC GM  48.553064
% ENT GM  1.066669
% LATEX   48.55 & 80.2     & 18.6     & 71.6     & 52.0    &
% LATEX   1.067 & 1.03     & 1.22     & 0.97     & 1.06    
% 
% INI experiments_configs/cifar10/ablations/class_nll_reg_55.ini
% ACC     79.4271
% ACC ERR 20.5729
% LATEX 20.57 &
% XCE     ECE       MCE       OVC       
% XCE     3.925514  20.299621 177.332296
% XCE GM  24.176300
% XCE GMO 24.176300
% LATEX 24.176 & 3.93 & 20.30 & 177.33 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     81.9550     16.1145     79.1472     54.9293     
% AUC ERR 18.0450     83.8855     20.8528     45.0707     
% ENT     0.0023      0.0014      0.0009      0.0034      
% AUC GM  48.950566
% ENT GM  0.001809
% LATEX   48.95 & 82.0     & 16.1     & 79.1     & 54.9    &
% LATEX   0.002 & 0.00     & 0.00     & 0.00     & 0.00
%
% INI feed_forward_resnet
% ACC     93.2392
% ACC ERR 6.7608
% LATEX 6.76 &
% XCE     ECE       MCE       OVC
% XCE     0.728364  40.611134 6.118503
% XCE GM  5.656469
% XCE GMO 5.656469
% LATEX 5.656 & 0.73 & 40.61 & 6.12 &
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet
% AUC     50.0000     50.0000     50.0000     50.0000
% AUC ERR 50.0000     50.0000     50.0000     50.0000
% ENT     0.3527      0.4365      0.1778      0.5107
% AUC GM  50.000000
% ENT GM  0.343835
% LATEX   50.00 & 50.0     & 50.0     & 50.0     & 50.0    &LATEX   0.344 & 0.35     & 0.44     & 0.18     & 0.51    &
% 
% INI VIB
% ACC     92.7083
% ACC ERR 7.2917
% LATEX 7.29 &
% XCE     ECE       MCE       OVC       
% XCE     0.680151  27.826962 4.706877  
% XCE GM  4.466155
% XCE GMO 4.466155
% LATEX 4.466 & 0.68 & 27.83 & 4.71 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     46.3716     52.1720     49.9728     41.6956     
% AUC ERR 53.6284     47.8280     50.0272     58.3044     
% ENT     0.3532      0.3840      0.1944      0.5175      
% AUC GM  47.383641
% ENT GM  0.341786
% LATEX   47.38 & 46.4     & 52.2     & 50.0     & 41.7    &LATEX   0.342 & 0.35     & 0.38     & 0.19     & 0.52    &
%
% INI i-RevNet
% ACC     90.9054
% ACC ERR 9.0946
% LATEX 9.09 &
% XCE     ECE       MCE       OVC       
% XCE     0.543417  14.780220 1.370198  
% XCE GM  2.224325
% XCE GMO 2.224325
% LATEX 2.224 & 0.54 & 14.78 & 1.37 & 
% DATASET rot_0.300   Qucikdraw   Noisy       ImageNet    
% AUC     50.0000     50.0000     50.0000     50.0000     
% AUC ERR 50.0000     50.0000     50.0000     50.0000     
% ENT     0.7433      0.8987      0.2542      0.8181      
% AUC GM  50.000000
% ENT GM  0.610501
% LATEX   50.00 & 50.0     & 50.0     & 50.0     & 50.0    &LATEX   0.611 & 0.74     & 0.90     & 0.25     & 0.82

==> illustrations/noise_amplification_tikz.tex <==
\newcommand{\ColorA}{RoyalBlue}
\newcommand{\ColorB}{ForestGreen}

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}
\pgfdeclarehorizontalshading{insideGradient}{10cm}{
                                                   color(0cm)=(white); 
                                                   color(2.6cm)=(white); 
                                                   color(3.3cm)=(\ColorA!50!white);
                                                   color(3.9cm)=(\ColorB!50!white);
                                                   color(4.4cm)=(white);
                                                   color(7cm)=(white)
                                                   }


\begin{tikzpicture}

    \filldraw[shading=insideGradient,draw=none] (0cm, 1.4cm) to[out=-6, in=210] (7cm, 3.7cm) -- (7cm, 1.8cm) to[in=6, out=195] (0cm, 0.8cm);
    \node [single arrow, 
           fill=black!15, draw=black, text=black,
           align=center, text width=4.5cm, minimum width=1.2cm, scale=0.90] at (3.5cm, 4.5cm) (model) {\textsf{\normalsize{\textbf{INN} $Z_\mathcal{E} = \INN(X + \mathcal{E})$}}};

    % X DOMAIN
    \begin{scope}

        % dotted x+eps line
        \draw[very thick, densely dotted, \ColorA!60, yshift=1.2cm] (0,0) -- (1cm,0);
        \node[text=\ColorA!60, scale=0.8] at (0.9, 1.4) {\small $X\!+\!\mathcal{E}$};

        % gauss curve
        \begin{axis}[
            no markers, domain=0:10, samples=300,
            axis line style={draw=none},
            height=3cm, width=5.3cm,
            xtick=\empty, ytick=\empty,
            enlargelimits=false, clip=false,
            rotate = -90
            ]
            \addplot [very thick,\ColorA] {gauss(7,0.3)};
        \end{axis}

        % sigma range
        \draw[thick, arrows=<->, yshift=0.75cm,xshift=-0.3cm] (0, 0) -- (0, 0.75cm) node [midway, left] {$\sigma$};

        % axis
        \node[text=black] at (0, 4.5cm) {$X$};
        \draw[very thick, arrows=->] (0,0) -- (0,4cm);
    \end{scope}


    % Z DOMAIN
    \begin{scope}[xshift=7cm]

        % dotted z_eps line
        \draw[very thick, densely dotted, \ColorB!60, yshift=2.85cm] (0,0) -- (1cm,0);
        \node[text=\ColorB!60, scale=0.8] at (0.9, 3.1) {\small $Z_\mathcal{E}$};

        % gauss curve
        \begin{axis}[
            no markers, domain=0:10, samples=300,
            axis line style={draw=none},
            height=3cm, width=5.3cm,
            xtick=\empty, ytick=\empty,
            enlargelimits=false, clip=false,
            rotate = -90
            ]
            \addplot [very thick,\ColorB] {gauss(3,0.8)};
        \end{axis}

        % sigma range
        \draw[thick, arrows=<->, yshift=1.7cm] (-0.3,0cm) -- (-0.3,1.8cm) node [midway, left] {$\sigma |J|$};

        % axis
        \node[text=black] at (0, 4.5cm) {$Z$};
        \draw[very thick, arrows=->] (0,0) -- (0,4cm);

    \end{scope}


\end{tikzpicture}
